Collaborative Video Diffusion: Consistent Multi-video Generation with Camera Control

Research on video generation has recently made tremendous progress, enabling high-quality videos to be generated from text prompts or images. Adding control to the video generation process is an important goal moving forward and recent approaches that condition video generation models on camera trajectories make strides towards it. Yet, it remains challenging to generate a video of the same scene from multiple different camera trajectories. Solutions to this multi-video generation problem could enable large-scale 3D scene generation with editable camera trajectories, among other applications. We introduce collaborative video diffusion (CVD) as an important step towards this vision. The CVD framework includes a novel cross-video synchronization module that promotes consistency between corresponding frames of the same video rendered from different camera poses using an epipolar attention mechanism. Trained on top of a state-of-the-art camera-control module for video generation, CVD generates multiple videos rendered from different camera trajectories with significantly better consistency than baselines, as shown in extensive experiments. Project page: https://collaborativevideodiffusion.github.io/.

==> sec/checklists.tex <==
\section*{NeurIPS Paper Checklist}

% %%% BEGIN INSTRUCTIONS %%%
% The checklist is designed to encourage best practices for responsible machine learning research, addressing issues of reproducibility, transparency, research ethics, and societal impact. Do not remove the checklist: {\bf The papers not including the checklist will be desk rejected.} The checklist should follow the references and precede the (optional) supplemental material.  The checklist does NOT count towards the page
% limit. 

% Please read the checklist guidelines carefully for information on how to answer these questions. For each question in the checklist:
% \begin{itemize}
%     \item You should answer \answerYes{}, \answerNo{}, or \answerNA{}.
%     \item \answerNA{} means either that the question is Not Applicable for that particular paper or the relevant information is Not Available.
%     \item Please provide a short (1–2 sentence) justification right after your answer (even for NA). 
%    % \item {\bf The papers not including the checklist will be desk rejected.}
% \end{itemize}

% {\bf The checklist answers are an integral part of your paper submission.} They are visible to the reviewers, area chairs, senior area chairs, and ethics reviewers. You will be asked to also include it (after eventual revisions) with the final version of your paper, and its final version will be published with the paper.

% The reviewers of your paper will be asked to use the checklist as one of the factors in their evaluation. While "\answerYes{}" is generally preferable to "\answerNo{}", it is perfectly acceptable to answer "\answerNo{}" provided a proper justification is given (e.g., "error bars are not reported because it would be too computationally expensive" or "we were unable to find the license for the dataset we used"). In general, answering "\answerNo{}" or "\answerNA{}" is not grounds for rejection. While the questions are phrased in a binary way, we acknowledge that the true answer is often more nuanced, so please just use your best judgment and write a justification to elaborate. All supporting evidence can appear either in the main paper or the supplemental material, provided in appendix. If you answer \answerYes{} to a question, in the justification please point to the section(s) where related material for the question can be found.

% IMPORTANT, please:
% \begin{itemize}
%     \item {\bf Delete this instruction block, but keep the section heading ``NeurIPS paper checklist"},
%     \item  {\bf Keep the checklist subsection headings, questions/answers and guidelines below.}
%     \item {\bf Do not modify the questions and only use the provided macros for your answers}.
% \end{itemize} 
 

% %%% END INSTRUCTIONS %%%


\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer:  \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: See abstract and Sec.~\ref{sec:intro}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A No or NA answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: See Sec.~\ref{sec:limitations}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper has no limitation while the answer No means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate "Limitations" section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory Assumptions and Proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: See Sec.~\ref{sec:supp_analysis}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental Result Reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: See Sec.~\ref{sec:experiments} and Sec.~\ref{sec:supp_details}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item If the paper includes experiments, a No answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and/or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We use public datasets and data processing details are provided in Sec.~\ref{sec:hybrid_training} and Sec.~\ref{sec:supp_details}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so “No” is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental Setting/Details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: See Sec.~\ref{sec:supp_details}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment Statistical Significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerNo{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Our evaluation uses protocols from previous works which do not use error bars.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The authors should answer "Yes" if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g. negative error rates).
        \item If error bars are reported in tables or plots, The authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments Compute Resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: See Sec.~\ref{sec:supp_details}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code Of Ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer No, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader Impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: See Sec.~\ref{sec:discussion}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that there is no societal impact of the work performed.
        \item If the authors answer NA or No, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNo{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification:
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We cited all works of codes and datasets used in the paper.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New Assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We do not release new assets.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset/code/model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and Research with Human Subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We do not conduct research with human subjects.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional Review Board (IRB) Approvals or Equivalent for Research with Human Subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Our paper does not involve research with human subjects.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\end{enumerate}


==> sec/old/method_old.tex <==
\section{Multi-View Videos Generation}
\label{sec:method}
Generally, video diffusion models (VDM) aim to generate a series of $N$ image frames $\bm{v}=\{\bm{x}^i, i\in 1,...,N\}$ by multiple denoising steps, given conditions such as text prompts or camera poses. With a data distribution $q_{\text{data}}(\bm{v})$, VDMs are commonly denoted as a reverse denoising function $p_\theta(\bm{v}_{t-1} | \bm{v}_{t}), t \in 1,...,T$ configured by learnable parameters $\theta$, where $T$ is the total denoising steps, to mimic the underlying reverse diffusion step $q(\bm{v}_{t-1} | \bm{v}_{t}, \bm{v}_{0})$ derived from the forward denoising process of the data. According to Ho et.al.\cite{ho2020ddpm}, the optimization of $p_\theta(\bm{v}_{t-1} | \bm{v}_{t})$ boils down to minimizing the following loss function:
\begin{equation}
    \mathcal{L}_{vdm} = \mathbb{E}_{\bm{\epsilon}, \bm{v}_0, t, c} \lVert \bm{\epsilon} - \bm{\epsilon}_\theta(\bm{v}_t, t, c)\rVert^2 ,
\end{equation}
where $\bm{v}_t$ is the noisy video generated from the data video $\bm{v}_0$ and random sampled Gaussian noise $\bm{\epsilon}$, $\bm{\epsilon}_\theta$ is the noise prediction model parameterized by $\theta$. $c$ is the condition of the generated video, which for example can be a text prompt (for text-to-video generation), a starting frame (for image-to-video generation), a camera trajectory (for camera-controlled video generation), or any combination of them. Alternatively, the learned function $\epsilon_\theta(\bm{v}_t, t, c)$ can also be treated as the (transformed) approximation of the score function $\nabla \log q(\bm{v}_t)$, according to the research of Song et.al.\cite{song2020score}

Empowered by the large-scale video datasets, many state-of-the-art VDMs~\cite{ho2022video, blattmann2023svd, brooks2024sora, guo2023animatediff, hu2023animateanyone, ho2022imagenvideo, esser2023gen1, blattmann2023alignyourlatents, ge2023pyoco} have successfully shown their ability to produce temporal consistent and realistic videos conditioned on certain inputs. One of the key drawbacks of all these existing methods, however, is the lack of consistency between multiple videos that are generated with the same condition. As Fig.~\ref{fig:videoconsensus} shows, videos generated with the same condition can be totally different in terms of contents and the overall spatial structure. This refrains the current VDMs from generating variant videos that shares the same structure or underlying 3D/4D geometries. One can simply use extended attention, for example, to increase the semantic similarities between the videos, yet this does not address the problem of structure consistency. In order to solve this problem, we introduce a novel objective for VDMs to generate multiple structural-consistent videos at the same time, same semantic condition, and dubbed it the generation of \textit{Video Consensus}. 

\begin{wrapfigure}{r}{0.6\textwidth}
    \centering
    \includegraphics[width=\linewidth]{fig/video_consensus.png}
    \caption{Illustration of video consensus. Existing video diffusion models generate videos separately, which may result in inconsistent frame contents (e.g. geometries, objects, motions) across videos (\textit{Left}); Video consensus generation aims to produce videos sharing the same underlying content (\textit{Right}). }
    \label{fig:videoconsensus}
    \vspace{-0.25cm}
\end{wrapfigure}

\subsection{Video Consensus}
Different from the original goal of video diffusion models, the generation of a video consensus seeks to find a set of $M$ videos $\bm{v}^i, i\in 1,...,M$, that comply with the unknown data distribution $q(\bm{v}^{1,...,M})$ given separate conditions $c_{1,...,M}$. In this setting, the target denoising function becomes $p_\theta(\bm{v}^{1,...,M} | c_{1,...,M})$, where $c_{1,...,M}$ are the conditions of all videos. One of the common examples of this task is to generate multi-view videos that are synchronously captured from the same dynamic 3D scene. In this setting, each video shares the same content (e.g. text prompt) but is conditioned on different camera trajectory.
% Similarly, the loss function for video consensus generation is:
% \begin{equation}
%     \mathcal{L}_{vc} = \mathbb{E}_{\bm{\epsilon}^{1,...,M}, \bm{v}^{1,...,M}_0, t, c} \lVert \bm{\epsilon}^{1,...,M} - \bm{\epsilon}_\theta(\bm{v}^{1,...,M}_t, t, c_{1,...,M})\rVert^2 .
% \end{equation}

In practice, however, directly training a model to generate multiple consensual videos is considerably intractable, mainly due to 1) The lack of datasets of correlated multiple videos and 2) The memory limitation of modern commercial GPUs. Inspired by the idea of factor graphs~\cite{loeliger2004introduction} in Graphical Models, we introduce an alternative approach to estimate the mutual distribution of all $M$ videos, by breaking down the generation of all $M$ videos into generating video subsets. Here, the denoising function for all $M$ videos is defined as: 
\begin{equation}
    p_\theta(\bm{v}^{1,...,M} | c_{1,...,M}) \ \dot\propto \ \mathcal{F} (\bm{p}), \text{where}  \ \bm{p} = \{ p_\theta(\bm{v}^S | c_S) \ | \ S \subset \{1,...,M\}\} 
\end{equation}
is the set of all marginal denoising functions defined on the subsets of $M$ videos, and $\mathcal{F}$ is a customized mapping function. This means the generated videos are set to be consistent within given subsets, instead of the whole set. Hence the score function of the mutual function $p_\theta(\bm{v}^{1,...,M} | c_{1,...,M})$ becomes:
\begin{align}
    & \nabla_{\bm{v}} \log p_\theta(\bm{v}^{1,...,M} | c_{1,...,M}) \ \\
    =& \nabla_{\bm{v}} \log \mathcal{F} (\exp (\log \bm{p})) \\
    =& \sum_{S} \frac{\partial \mathcal{F'}}{\partial \log p_\theta(\bm{v}^S | c_{S})} \cdot \nabla_{\bm{v}}\log p_\theta(\bm{v}^{S} | c_{S}). \quad (\mathcal{F}' = \log \ \circ \ \mathcal{F} \circ \exp) \\
    \label{eq:origin} \dot=& \sum_{S}  J_{\mathcal{F'}}(S) \cdot \nabla_{\bm{v}}\log p_\theta(\bm{v}^{S} | c_{S}). 
\end{align}

Where $\circ$ is the function composition operator. This implies that the mutual score function of all videos can be represented by the weighted sum of subset score functions. We prove in the supplementary that the defined $p_\theta(\bm{v}^{1,...,M} | c_{1,...,M})$ is able to estimate the unknown data distribution derived from the forward diffusion process $q(\bm{v}^{1,...,M} | c_{1,...,M})$, only when $\sum_{S}\bm{1}(k\in S) J_\mathcal{F'}(S)=1$ for all $k\in 1,...,M$. 
Naively, one can define $\mathcal{F}(\bm{p}) = C\cdot \prod_{i} p_\theta(\bm{v}^i | c_{i})^{1/M} $, where $C$ is a normalizing constant. In this case, the mutual denoising function collapses to the original function in the VDMs, which predicts each video individually and has no interaction with cross-view knowledge.
Observing that the consistency between $M$ videos together can be practically treated as the consistency between all video pairs, in this work we seek to build the video consensus from consistent video pairs, by defining our mapping function as  $\mathcal{F}_{pair}(\bm{p}) = \mathcal{F}(\{p_\theta(\bm{v}^{i,j} | c_{i,j}) \ | \ i,j\in 1,...,M\})$. 
% $\mathcal{F}_{pair}(\bm{p}) = C \cdot \prod_{i\neq j} p_\theta(\bm{v}^{i,j} | c_{i,j})^{1/M(M-1)}$. 
% which corresponds to taking the average of all score functions defined on video pairs $\bm{v}^{i,j}$ during the . 
% \begin{equation}
%     \nabla_{\bm{v}_t} \log p_\theta(\bm{v}^{1,...,M} | c_{1,...,M}) \ 
%     = \sum_{j\neq t} \frac{\nabla_{\bm{v}_t} p_\theta(\bm{v}^{t,j} | c_{t,j})}{ p_\theta(\bm{v}^{t,j} | c_{t,j})} 
%     = \sum_{j\neq t} \nabla_{\bm{v}_t} \log p_\theta(\bm{v}^{t,j} | c_{t,j}),
% \end{equation}
In this case, given a dataset of paired videos representing the distribution $q_{data} (\bm{v}^{i,j} | c_{i,j})$, we train our pairwise denoising function $p_{\theta} (\bm{v}^{i,j} | c_{i,j})$ with the following updated diffusion loss:
\begin{equation}
    \mathcal{L}_{vc} = \mathbb{E}_{i, j, \bm{\epsilon}^{i,j}, \bm{v}^{i,j}_0, t, c} \lVert \bm{\epsilon}^{i,j} - \bm{\epsilon}_\theta(\bm{v}^{i,j}_t, t, c_{i,j})\rVert^2.
\end{equation}
Next, we explain how our model is built and trained.

%$p_\theta(\bm{v}^{i,j}_{t-1} | \bm{v}^{i,j}_{t}, c_{i,j})$, is a joint denoising function of two videos $v_i, v_j$ that learned from $q_{data}(v^{i,j})$

\section{EpiCtrl}
\begin{figure}[t]
  \centering
  \includegraphics[width=\textwidth]{fig/Method.pdf}
  \caption{Our method: Left: synchronization module, Right: Two-phase training}
  \label{fig:epictrl}
\end{figure}

\begin{wrapfigure}{r}{0.5\textwidth}
    \centering
    \includegraphics[width=\linewidth]{fig/Hybrid_training.pdf}
    \caption{Two-Phase Hybrid Training.}
    \label{fig:hybridtraining}
    \vspace{-0.25cm}
\end{wrapfigure}


Inspired by ~\cite{he2024cameractrl, guo2023animatediff}, we opt to build our model EpiCtrl as an extension of the camera-controlled video model CameraCtrl~\cite{he2024cameractrl}. 
Our model is trained to generate two videos $\bm{v}^{i,j}$ at one time, given the same text prompt $y$ and two different camera trajectories $cam^{i,j}_{1,...,N}$. To ease the generation of consistent videos, we assume the two videos are synchronized (i.e. frames for the videos are captured at the same time), and the first pose of two trajectories $cam^{i,j}_1$ are set to be identical, forcing the first frame of two videos to be the same. 

As shown in Fig.~\ref{fig:epictrl}, our model takes two noisy input videos and generate the noise prediction in a single pass. The two videos share the same pretrained weights of CameraCtrl, and are synchronized in our proposed \textit{Cross-View Synchronization Modules}, which are explained Sec.~\ref{sec:cross_view_module}. The model is trained with two different datasets, RealEstate10K~\cite{zhou2018realestate10k} and WebVid10M~\cite{bain2021webvid}. The first dataset consists of camera-calibrated video on mostly static scenes, and the second contains  generic videos without poses. This leads to our two-phase training strategy, which will be introduced in Sec.~\ref{sec:hybrid_training}. The learned model is able to infer arbitrary numbers of multi-view videos using our proposed inference algorithm, which will be explained in Sec.~\ref{sec:multiview}.

\subsection{Cross-View Synchronization Module}
\label{sec:cross_view_module}
To this day, state-of-the-art video diffusion models commonly incorporate variant types of attention mechanisms defined on the spatial and temporal dimension: many works such as AnimateDiff~\cite{guo2023animatediff}, SVD~\cite{blattmann2023svd}, LVDM~\cite{he2022lvdm} disentangles space and time and applies separate attention layers; the very recent breakthrough SORA~\cite{brooks2024sora} processes both dimension jointly on its 3D spatial-temporal attention modules. Whilst the operations defined on the spatial and temporal dimensions together bring strong correlation between different pixels of different frames, capturing the context between different videos requires a new operation to be added: cross-video attention. Thankfully, many works \zhengfei{cite} have shown that the so called extended attention technique, i.e. concatenating the key and values from different views together, is evidently efficient for preserving identical semantic information across videos. However, it refrains from preserving the structure consistency among them, leading to totally different scenes in terms of geometry. Thus, inspired by the previous work~\cite{tseng2023poseguideddiffusion}, we introduce the \textit{Cross-View Synchronization Module} based on the epipolar geometry, to shed light on the structure relationship between cross-video frames during the generation process, aligning the video pair towards the same geometry. 

Fig.~\ref{fig:epictrl} demonstrates the design of our cross-view module. Taking a pair of latent map sequences $z^i_{1,..,N}, z^j_{1,..,N}$ as input, our module applies a cross-video attention between the same frames from the two videos. Specifically, we adapt the epipolar attention design from Tseng et.al.~\cite{tseng2023poseguideddiffusion} and define our module as:
\begin{align}
    & out^i_k = \text{ff}(\text{Attn}(W_Q z^i_k, W_K z^j_k, W_V z^j_k, \mathcal{M}^{i,j}_k)), \quad \forall k\in1,...,N, \\
    & \mathcal{M}^{i,j}_k(x_i, x_j) = 
    \bm{1}(x_j^TF_k^{i\rightarrow j}x_i<\tau_{\text{epi}})
\end{align}
where $W_Q, W_K, W_V$ are the query, key, value mapping matrices, $\mathcal{M}$ is the attention mask, $\text{Attn}(Q, K, V, \mathcal{M})$ is the  attention operator introduced from the Transformer~\cite{vaswani2017attention}, ff is the feed-forward function and $F_k^{i\rightarrow j}$ is the fundamental matrix between $cam^i_{k}$ and $cam^j_{k}$. $\tau_{\text{epi}}$ is set to $3$ in all of our experiments.
The key insight of this module is that, as the two videos are assumed to be synchronized to each other, the same frame from the two videos is supposed to share the same underlying geometry, and hence can be correlated by their epipolar geometry defined by the given camera poses. For the first frames where the camera poses are set to be identical since the fundamental matrix is undefined here, we generate pseudo epipolar lines for each pixel with random slopes that go through the pixels themselves. We show in our study that the epipolar-based attention remarkably increases the geometry integrity of the generated video pairs.

\subsection{Hybrid Training Strategy from Two Datasets}
\label{sec:hybrid_training}
Preferably, one can directly train the model on any dataset consisting of camera-registered video pairs. We, however, opt to not train the model in this way, due to the lack of such dataset captured from the real world in large scale. Alternatively, we make use of the two popular monocular datasets, RealEstate10K~\cite{zhou2018realestate10k} and Webvid10M~\cite{bain2021webvid}, to develop a hybrid training strategy for video pair generation models. 

\paragraph{RealEstate10K with Video Folding.}
The first phase of the training involves with RealEstate10K~\cite{zhou2018realestate10k}, a dataset consists of video clips captured mostly in static scenes (e.g. indoor layouts), and corresponding camera poses. Assuming that it is reasonable to reverse a video captured in static scenes, we sample video pairs by simply sampling subsequences of $2M-1$ frames from a video in the dataset, then cutting them from the middle and reversing their first parts to form synchronized video pairs (In other words, the subsequences are folded into two video clips).

\paragraph{Webvid10M with Homography Augmentation.}
While RealEstate10K provides good information about geometry transformations, training our model merely on it is not an ideal option, since it does not provides any knowledge on motions and only contains estate scenes. 

On the other hand, Webvid10M being a large-scale video dataset consists of all kinds of videos, and can be used as a good supplement of RealEstate10K. Here, to extract video pairs, we simply clone the videos in the dataset, then apply random homography transformations to the clones. Nonetheless, The Webvid10M dataset does not contain any camera information, making it unsuitable for camera-conditioned model training. To address this problem, we propose a two-phase training strategy to adapt both datasets (with or without camera poses) for the same model. 

\paragraph{Two-Phase Training.}
As previously mentioned, our model is built upon the existing camera-controlled video diffusion model CameraCtrl\cite{he2024cameractrl}. CameraCtrl, similarly, is an extended version of the video diffusion model AnimateDiff\cite{guo2023animatediff}, by adding a pose encoder and several pose feature injectors for the temporal attention layers to the original model. Both of these models, are based on the fundamental image diffusion model Stable Diffusion \cite{rombach2022latentdiffusion}. 
This brings to the assumption that both of these models incorporate with the same domain of latent space, and thus it is possible to train a universal module that can be adapted by all of them. Therefore, our training scheme is designed as the Fig.~\ref{fig:hybridtraining} shows: for the RealEstate10K dataset, we use CameraCtrl with LORA fine-tuned on RealEstate10K as the backbone, and apply the ground truth epipolar geometry in the cross-video module; And for the Webvid10M dataset, we use AnimateDiff with LORA fine-tuned on Webvid10M as the backbone, and apply the pseudo epipolar geometry (the same one used for the first frames in RealEstate10K dataset) in the cross-video module. In our experiment, this hybrid training strategy greatly helps the model to generate videos with both synchronized motions and great geometry consistency.

\subsection{Toward Multi-View Video Generation}
\label{sec:multiview}
As mentioned in Sec.~\ref{sec:method}, given the trained video pair generation model, we aim to generate multiple videos that share consistent contents and motions. At each denoising step, one feed the pair video model with all possible pairs (every $\bm{v}^{i,j}$, where $i,j\in 1,...M, i\neq j$), then average the output noises to get the final noise prediction. This strategy, being equivalent to defining $\mathcal{F}_\text{pair}(\bm{p}) = C\cdot \prod_{i,j} p_\theta(\bm{v}^{i,j} | c_{i,j})^{1/M(M-1)}$, has two major drawbacks: 1) The computational complexity is $O(M^2)$, which is considerably high and 2) We empirically find that averaging the predicted noises   smooths out high frequency details in the results. To improve this exhaustive method, we embrace the idea introduced by Bansal et.al.~\cite{bansal2023universal}, and designed a novel randomized algorithm with recurrent denoising steps. Specifically, at each denoising step $t$, We repeat the following the process in multiple iterations: We randomly arrange $M$ noisy video inputs into $\frac{M}{2}$ pairs, use the network to inference their noise predictions, denoise the inputs to the $t-1$'s noise level, and finally add a random noise back to the $t$'s noise level unless it is the last iteration. This randomized recurrent algorithm effectively reduced the calculation workload while preserving multi-view consistency as well. More details of the algorithm will be demonstrated in our supplementary.

==> sec/old/method_old_2.tex <==
\section{Multi-View Videos Generation}
\label{sec:method}
Conventionally, video diffusion models (VDMs) aim to generate videos from randomly sampled Gaussian noise with multiple denoising steps, given conditions such as text prompts, frames, or camera poses. 
Specifically, let $\bm{v}_0\sim q_{\text{data}}(\bm{v})$ be a data point sampled from the data distribution, the forward diffusion process continuously adds noises to $\bm{v}_0$ to get a series of $\bm{v}_t, t\in1,...,T$ until it becomes Gaussian noise. Using the reparameterization trick from Ho et al.\cite{ho2020ddpm}, the distribution of $\bm{v}_t$ can be represented as $q(\bm{v}_t\ | \ \bm{v}_0) = \mathcal{N}(\bm{v}_t; \ \sqrt{\bar\alpha_t}\bm{v}_0, (1-\bar\alpha_t) I)$, where $\bar\alpha_t \in (0, 1]$ are the noise scheduling parameters, which are monotonously increasing, and $\bar\alpha_T=1$. The video diffusion model, typically denoted as $p_\theta(\bm{v}_{t-1} | \bm{v}_{t})$, is a model parameterized by $\theta$ that is trained to estimate the backward distribution $q(\bm{v}_{t-1} | \bm{v}_{t}, \bm{v}_{0})$. According to Ho et al.\cite{ho2020ddpm}, the optimization of $p_\theta(\bm{v}_{t-1} | \bm{v}_{t})$ boils down to minimizing the following loss function:
\begin{equation}
    \mathcal{L}_{vdm} = \mathbb{E}_{\bm{\epsilon}, \bm{v}_0, t, c} \lVert \bm{\epsilon} - \bm{\epsilon}_\theta(\bm{v}_t, t, c)\rVert^2 ,
\end{equation}
where $\bm{v}_t = \sqrt{\bar \alpha_t} \bm{v}_0+(1-\bar \alpha_t)\bm{\epsilon}$ is the noisy video generated from $\bm{v}_0$ and a random sampled Gaussian noise $\bm{\epsilon}$, $\bm{\epsilon}_\theta(\bm{v}_t, t)$ is the noise prediction of the VDM, and $c$ is the video condition. During inference time, one can start from a normalized Gaussian noise $\bm{v}_T\sim \mathcal{N}(0, I)$ and apply the noise prediction model $\bm{\epsilon}_\theta(\bm{v}_t, t)$ multiple times to denoise it until $\bm{v}_0$.
%Alternatively, the learned function $\epsilon_\theta(\bm{v}_t, t, c)$ can also be treated as the (transformed) approximation of the score function $\nabla \log q(\bm{v}_t)$, according to the research of Song et al.\cite{song2020score}

Empowered by readily available large-scale video datasets, many state-of-the-art VDMs~\cite{ho2022video, blattmann2023svd, brooks2024sora, guo2023animatediff, hu2023animateanyone, ho2022imagenvideo, esser2023gen1, blattmann2023alignyourlatents, ge2023pyoco} have successfully shown their ability to produce temporally consistent and realistic videos conditioned on certain inputs. However, one of the key drawbacks of all these existing methods is the lack of consistency between multiple videos generated with the same condition. As Fig.~\ref{fig:videoconsensus} shows, videos generated with the same condition can be totally different in terms of contents and the overall spatial structure. This hinders current VDMs from generating variant videos that share the same structure or underlying 3D/4D geometries. One can use inference-stage tricks such as extended attention~\cite{cai2023genren} to increase the semantic similarities between the videos, yet this does not address the problem of structure consistency. To address this issue, we introduce a novel objective for VDMs to generate multiple structurally consistent videos simultaneously given certain semantic conditions and dub it collaborative video diffusion. %the generation of \textit{Video Consensus}.

\input{fig/video_consensus}
\subsection{Collaborative Video Diffusion}
In contrast to conventional video diffusion models, \method{} seeks to find an arbitrary number of videos $\bm{v}^i, i\in 1,...,M$ that comply with the unknown data distribution $q_\text{data}(\bm{v}^{1,...,M})$ given separate conditions $c_{1,...,M}$. Similarly, the collaborative video diffusion model can be represented as $p_\theta(\bm{v}^{1,...,M} | c_{1,...,M})$. An examples includes multi-view videos synchronously captured from the same dynamic 3D scene. % or videos in different art styles but with the same content. %-> we don't show this, so don't motivate it 

In practice, however, directly training a model to generate multiple consistent videos is intractable because of 1) a lack of large-scale multi-view video training data and 2) the limited memory provided by commercial GPUs. 
Observing that the consistency between $M$ videos together can be practically treated as the consistency between all video pairs, in this work, we seek to collaboratively generate consistent videos from a model trained on video pairs $\bm{v}^{i,j}$.

In general, given a dataset of paired videos representing the distribution $q_{data} (\bm{v}^{i,j} | c_{i,j})$, a pairwise denoising function $p_{\theta} (\bm{v}^{i,j} | c_{i,j})$ can be trained with the following updated diffusion loss:
\begin{equation}
    \mathcal{L}_{pair} = \mathbb{E}_{i, j, \bm{\epsilon}^{i,j}, \bm{v}^{i,j}_0, t, c} \lVert \bm{\epsilon}^{i,j} - \bm{\epsilon}_\theta(\bm{v}^{i,j}_t, t, c_{i,j})\rVert^2.
\end{equation}
Using this model, we are able to propose several strategies to assemble the predicted noises on video pairs into the noise prediction of all $M$ videos, and eventually generate $M$ consensual videos with the same denoising pipeline that is used in VDMs. A more detailed mathematical analysis of this video pair based consensus generation is provided in our supplementary to further explain our idea. 

In the next section, we will explain the major steps in preparing our dataset, building our model, and designing our algorithms for video consensus generation. 

\section{Collaborative Video Diffusion with Camera Control}
\begin{figure}[t]
  \centering
  \includegraphics[width=\textwidth]{fig/Method.pdf}
  \caption{\textbf{Architecture of collaborative video diffusion}. \textit{Left}: The model takes two (or more) noisy video features and camera pose trajectories as input and generates the noise prediction for both videos. Note that the image autoencoder of Stable Diffusion is omitted here; \textit{Right}: A closer look of our \textit{Cross-View Synchronization Module}, which takes the same frames from the two videos along with the corresponding fundamental matrix as input, and applies a masked cross-view attention between the frames.}
  \label{fig:epictrl}
\end{figure}

In our work, we aim to generate $M$ consistent videos given a universal text prompt $y$ and $M$ individual camera trajectories $cam^{1,...,M}$. Analogously, our diffusion model is trained to generate two videos $\bm{v}^{i,j}$ given the same text prompt $y$ and two camera trajectories $cam^{i,j}$.
To ease the generation of consistent videos, we assume the two videos are synchronized (i.e., frames for the videos are captured simultaneously) and set the first pose of every trajectory to be identical, forcing the first frame of all videos to be the same.

Inspired by ~\cite{he2024cameractrl, guo2023animatediff}, our model is designed as an extension of the camera-controlled video model CameraCtrl~\cite{he2024cameractrl}. As shown in Fig.~\ref{fig:epictrl}, our model takes two noisy video inputs and generates the noise prediction in a single pass. The two videos share the same pretrained weights of CameraCtrl and are synchronized in our proposed \textit{Cross-View Synchronization Modules} (Sec.~\ref{sec:cross_view_module}). The model is trained with two different datasets: RealEstate10K~\cite{zhou2018realestate10k}, which consists of camera-calibrated video on mostly static scenes, and WebVid10M~\cite{bain2021webvid}, which contains generic videos without poses. This leads to our two-phase training strategy introduced in Sec.~\ref{sec:hybrid_training}. The learned model can infer arbitrary numbers of videos using our proposed inference algorithm, which will be described in Sec.~\ref{sec:multiview}.

\subsection{Cross-View Synchronization Module}
\label{sec:cross_view_module}
Current state-of-the-art VDMs commonly incorporate various types of attention mechanisms defined on the spatial and temporal dimension: works such as AnimateDiff~\cite{guo2023animatediff}, SVD~\cite{blattmann2023svd}, LVDM~\cite{he2022lvdm} disentangles space and time and applies separate attention layers; the very recent breakthrough SORA~\cite{brooks2024sora} processes both dimensions jointly on its 3D spatial-temporal attention modules. Whilst the operations defined on the spatial and temporal dimensions bring a strong correlation between different pixels of different frames, capturing the context between different videos requires a new operation: cross-video attention. Thankfully, prior works~\cite{ceylan2023pix2video, cai2023genren} have shown that the extended attention technique, i.e., concatenating the key and values from different views together, is evidently efficient for preserving identical semantic information across videos. However, it refrains from preserving the structure consistency among them, leading to totally different scenes in terms of geometry. Thus, inspired by the previous work~\cite{tseng2023poseguideddiffusion}, we introduce the \textit{Cross-View Synchronization Module} based on the epipolar geometry to shed light on the structure relationship between cross-video frames during the generation process, aligning the video pair towards the same geometry. 

Fig.~\ref{fig:epictrl} demonstrates the design of our cross-view module. Taking a pair of feature sequences $\mathbf{z}^i_{1,..,N}, \mathbf{z}^j_{1,..,N}$ of $N$ frames as input, our module applies a cross-video attention between the same frames from the two videos. Specifically, we adapt the epipolar attention design from Tseng et al.~\cite{tseng2023poseguideddiffusion} and define our module as:
% \begin{align}
%     & out^i_k = \text{ff}(\text{Attn}(W_Q z^i_k, W_K z^j_k, W_V z^j_k, \mathcal{M}^{i,j}_k)), \quad \forall k\in1,...,N, \\
%     & \mathcal{M}^{i,j}_k(x_i, x_j) = 
%     \bm{1}(x_j^TF_k^{i\rightarrow j}x_i<\tau_{\text{epi}})
% \end{align}
\begin{align}
    & out^i_k = \texttt{ff}(\texttt{Attn}(\mathbf{W}_Q \mathbf{z}^i_k, \mathbf{W}_K \mathbf{z}^j_k, \mathbf{W}_V \mathbf{z}^j_k, \mathcal{M}^{i,j}_k)), \quad \forall k\in1,...,N, \\
    & \mathcal{M}^{i,j}_k(\mathbf{x}_i, \mathbf{x}_j) = 
    \bm{1}(\mathbf{x}_j^T\mathbf{F}_k^{i\rightarrow j}\mathbf{x}_i<\tau_{\text{epi}})
\end{align}
where $k$ is the frame index, $\mathbf{W}_Q, \mathbf{W}_K, \mathbf{W}_V$ are the query, key, value mapping matrices, $\mathcal{M}$ is the attention mask, $\texttt{Attn}(Q, K, V, \mathcal{M})$ is the  attention operator introduced from the Transformer~\cite{vaswani2017attention}, $\texttt{ff}$ is the feed-forward function and $\mathbf{F}_k^{i\rightarrow j}$ is the fundamental matrix between $cam^i_{k}$ and $cam^j_{k}$. $\tau_{\text{epi}}$ is set to $3$ in all of our experiments.
The key insight of this module is as the two videos are assumed to be synchronized to each other, the same frame from the two videos is supposed to share the same underlying geometry and hence can be correlated by their epipolar geometry defined by the given camera poses. For the first frames where the camera poses are set to be identical since the fundamental matrix is undefined here, we generate pseudo epipolar lines for each pixel with random slopes that go through the pixels themselves. Our study shows that epipolar-based attention remarkably increases the geometry integrity of the generated video pairs.

\subsection{Hybrid Training Strategy from Two Datasets}
\label{sec:hybrid_training}
Ideally, one can directly train the model on any dataset consisting of camera-registered video pairs. However, this is extremely challenging due to the lack of such a large-scale real-world dataset. Alternatively, we opt to make use of the two popular monocular datasets, RealEstate10K~\cite{zhou2018realestate10k} and Webvid10M~\cite{bain2021webvid}, to develop a hybrid training strategy for video pair generation models. 
\begin{wrapfigure}{r}{0.5\textwidth}
    \centering
    \includegraphics[width=\linewidth]{fig/Hybrid_training.pdf}
    \caption{\textbf{Two-Phase Hybrid Training.} We use different data processing schemes to handle the two datasets (\textit{Top}) and apply separate model structures to train in corresponding phases (\textit{Bottom}).}
    \label{fig:hybridtraining}
    \vspace{-0.25cm}
\end{wrapfigure}
\paragraph{RealEstate10K with Video Folding.}
The first phase of the training involves RealEstate10K~\cite{zhou2018realestate10k}, a dataset consisting of video clips capturing mostly static indoor scenes and corresponding camera poses. We sample video pairs by simply sampling subsequences of $2M-1$ frames from a video in the dataset, then cutting them from the middle and reversing their first parts to form synchronized video pairs. In other words, the subsequences are folded into two video clips.

\paragraph{Webvid10M with Homography Augmentation.}
While RealEstate10K~\cite{zhou2018realestate10k} provides decent geometry prior, training our model merely on itself is not ideal since it does not provide any knowledge regarding dynamics and only contains indoor scenes. 
On the other hand, Webvid10M, a large-scale video dataset, consists of all kinds of videos and can be used as a good supplement to RealEstate10K. To extract video pairs, we clone the videos in the dataset and then apply random homography transformations to the clones. Nonetheless, The Webvid10M dataset contains no camera information, making it unsuitable for camera-conditioned model training. To address this problem, we propose a two-phase training strategy to adapt both datasets (with or without camera poses) for the same model.

\paragraph{Two-Phase Training.}
As previously mentioned, our model is built upon the existing camera-controlled VDM CameraCtrl~\cite{he2024cameractrl}. It is an extended version of AnimateDiff~\cite{guo2023animatediff} by adding a pose encoder and several pose feature injectors for the temporal attention layers to the original model. Both AnimateDiff~\cite{guo2023animatediff} and CameraCtrl~\cite{he2024cameractrl} are based on Stable Diffusion \cite{rombach2022latentdiffusion}.
This implies that they incorporate the same latent space domain, and thus, it is feasible to train a module that can be universally adapted. Therefore, as Fig.~\ref{fig:hybridtraining} shows, our training scheme is designed as: for the RealEstate10K dataset, we use CameraCtrl with LORA fine-tuned on RealEstate10K as the backbone and applying the ground truth epipolar geometry in the cross-video module; For the Webvid10M dataset, we use AnimateDiff with LORA fine-tuned on Webvid10M as the backbone, and apply the pseudo epipolar geometry (the same strategy used for the first frames in RealEstate10K dataset) in the cross-video module. Experiments show that the hybrid training strategy greatly helps the model generate videos with synchronized motions and great geometry consistency.

\subsection{Towards More Videos}
\label{sec:multiview}
Using the trained video pair generation model, we can generate multiple videos that share consistent content and motions. At each denoising step, we select $P$ video pairs $\mathcal{P}=\{\bm{v}^{i_1,j_1}, \bm{v}^{i_2,j_2}, ..., \bm{v}^{i_P,j_P}\}$ among all $M$ videos, then use the trained network for noise prediction of each pair, and averaging them w.r.t. each video. That is, the output noise for $k$th video is defined as: $\bm{\epsilon}_{out}(\bm{v}^i_t) = \text{Avg}_{\bm{v}^{i,j} \in \mathcal{P}} (\bm{\epsilon}^i_\theta(\bm{v}^{i,j}_t, t, cam^{i,j}))$, where $\bm{\epsilon}^i_\theta(\bm{v}^{i,j}_t, t, cam^{i,j})$ is the noise prediction for $\bm{v}^i_t$ given the video pair input $\bm{v}^{i,j}_t$.
For pair selection, we propose the following strategies:
\begin{itemize}
\item \textit{Exhaustive Strategy}: Select all $M(M-1)/2$ pairs. 
\item \textit{Partition Strategy}: Randomly divide $M$ noisy video inputs into $\frac{M}{2}$ pairs. 
\item \textit{Multi-Partition Strategy}: Repeat the Partition Strategy multiple times and concatenate all pairs.
\end{itemize}
The exhaustive strategy has a higher computational complexity of $O(M^2)$ compared to the partition one ($O(M)$) but covers every pair among $M$ videos and thus can produce more consistent videos. The multi-partition strategy, on the other hand, is a trade-off between the two strategies. We also embrace the recurrent denoising method introduced by Bansal et al.~\cite{bansal2023universal} that do multiple recurrent iterations on each denoising timestep. 
We provide the pseudo-code of our inference algorithm and more analysis in our supplementary.
%That is, at each denoising step $t$, we repeat the following the process in multiple iterations: We infer the noise prediction of all videos using one of the two strategies, denoise the inputs to the $t-1$'s noise level, and add a random noise back to the $t$'s noise level unless it is the last iteration. 
